Hybrid Handcrafted and Learnable Audio Representation for Analysis of Speech Under Cognitive and Physical Load

As a neurophysiological response to threat or adverse conditions, stress can affect cognition, emotion and behaviour with potentially detrimental effects on health in the case of sustained exposure. Since the affective content of speech is inherently modulated by an individual's physical and mental state, a substantial body of research has been devoted to the study of paralinguistic correlates of stress-inducing task load. Historically, voice stress analysis (VSA) has been conducted using conventional digital signal processing (DSP) techniques. Despite the development of modern methods based on deep neural networks (DNNs), accurately detecting stress in speech remains difficult due to the wide variety of stressors and considerable variability in the individual stress perception. To that end, we introduce a set of five datasets for task load detection in speech. The voice recordings were collected as either cognitive or physical stress was induced in the cohort of volunteers, with a cumulative number of more than a hundred speakers. We used the datasets to design and evaluate a novel self-supervised audio representation that leverages the effectiveness of handcrafted features (DSP-based) and the complexity of data-driven DNN representations. Notably, the proposed approach outperformed both extensive handcrafted feature sets and novel DNN-based audio representation learning approaches.

==> IEEEtran/tools/README <==

January 11, 2007


The IEEEtrantools.sty package provides several commands from the
IEEEtran.cls file so that they can be used under other LaTeX classes. The
user guide provided here covers only the differences in the use of the
commands from those provided by IEEEtran.cls. For complete documentation
on these commands, see the relevant sections in the IEEEtran_HOWTO manual
of the IEEEtran LaTeX class.

The IEEEtrantools.sty package provides the following IEEEtran.cls commands:

 1. \IEEEPARstart which produces large initial "drop cap" letters.
 2. the \bstctlcite command for the control entry types of IEEEtran.bst
    V1.00 and later
 3. the IEEE itemize, enumerate and description list environments
 4. the complete IEEEeqnarray family for producing multiline equations
    as well as matrices and tables, including the IEEEeqnarray support
    commands.

IEEEtrantools.sty should not be used with IEEEtran.cls.

For helpful tips, answers to frequently asked questions and other support,
visit the IEEEtrantools support page at my website:

http://www.michaelshell.org/tex/ieeetran/tools/


Enjoy!

Michael Shell
http://www.michaelshell.org/


*******
1/2007 V1.2 (V1.7 of IEEEtran.cls) changes:

 1. Several commands and enviroments have depreciated in favor of
    replacements with IEEE prefixes to better avoid potential future name
    clashes with other packages. Legacy code retained to allow use of the
    obsolete forms, but with an warning message to the console during
    compilation:
    \IEEEPARstart
    For IED lists:
    \IEEEiedlabeljustifyc, \IEEEiedlabeljustifyl, \IEEEiedlabeljustifyr,
    \IEEEnocalcleftmargin, \IEEElabelindent, \IEEEsetlabelwidth,
    \IEEEusemathlabelsep
 
 2. These commands/lengths now require the IEEE prefix and do not have
    legacy support: \IEEEnormaljot.
    For IED lists: \ifIEEEnocalcleftmargin, \ifIEEEnolabelindentfactor,
    \IEEEiedlistdecl, \IEEElabelindentfactor

 3. \normalsizebaselineskip no longer provided. 

 4. New \IEEEPARstart controls:
    \IEEEPARstartHEIGHTTEXT, \IEEEPARstartFONTSTYLE, \IEEEPARstartCAPSTYLE,
    \IEEEPARstartWORDFONTSTYLE, \IEEEPARstartWORDCAPSTYLE,
    \IEEEPARstartHOFFSET, \IEEEPARstartITLCORRECT
    and the (output) length \IEEEPARstartletwidth.

 5. Provide for an optional argument to \bstctlcite to provide a way to
    specify a different aux file. Define \bstctlcite even if it has already
    been defined.

********************************** Files **********************************

README                - This file.

IEEEtrantools.sty     - The LaTeX package file.

IEEEtrantools_doc.txt - The user manual - supplementary to the 
                        IEEEtran_HOWTO manual.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtrantools.sty, IEEEtrantools_doc.txt
***************************************************************************



==> Table2_with_WM.tex <==
\begin{table*}[h!]
  \centering
  \caption{Test
  UAR (\%) on cognitive and physical load datasets. \{\} indicates concatenation of feature vectors. OS: openSMILE~\cite{eyben2010opensmile}. The best scores are shown in bold. UM: unweighted mean, WM: mean weighted by dataset size.}
  \vspace{-6pt}
  \begin{tabular}{lccccc@{\hspace{20pt}}cc}
\toprule
Model & Cog1 & Cog2 & Cog3 & Cog4 & Phys & UM & WM\\
\midrule
VGGish\cite{hershey2017}                                                                                             & 64.0   & 69.6 & 90.0   & 77.1 & 55.0 & 71.1 & 73.7 \\
TRILL, layer 19\cite{shor2020}                                                                                       & 58.8 & 72.9 & 93.3 & 74.0   & 62.5 & 72.3 & 74.9 \\
OS/eGeMAPS\cite{eyben2015geneva}                                                                                     & 62.9 & 65.4 & 93.8 & 72.9 & 67.5 & 72.5 & 74.1 \\
BYOL-A\cite{niizumi2021byol}                                                                                         & 68.0   & 70.4 & 90.0   & 81.3 & 61.3 & 74.2 & 75.9 \\
YAMNet\cite{plakal2020}                                                                                              & 58.1 & 71.7 & 99.2 & 83.3 & 62.5 & 75.0 & 77.2 \\
BYOL-S\cite{scheidwasser2021serab}                                                                                   & 65.3 & 72.9 & 91.7 & 80.2 & 66.3 & 75.3 & 76.9 \\
OS/ComParE\cite{eyben2010opensmile}                                                                                  & 78.7 & 74.6 & \textbf{100.0}  & 79.2 & 52.5 & 77.0 & 81.0 \\
BYOL-S/CvT\cite{scheidwasser2021serab}                                                                               & 79.2 & \textbf{80.0}   & \textbf{100.0}  & 74.0   & 57.5 & 78.1 & 82.5 \\
\midrule
\textbf{\textit{Hybrid \& ensemble models:}} \\
\{BYOL-S\cite{scheidwasser2021serab};   OS/ComParE\cite{eyben2010opensmile}\}     & 76.2 & 77.9 & \textbf{100.0}  & 83.3 & 56.3 & 78.7 & 82.3 \\
\{BYOL-S/CvT \cite{scheidwasser2021serab};   OS/ComParE\cite{eyben2010opensmile}\} & 81.2 & 77.1 & \textbf{100.0}  & 79.2 & 57.5 & 79.0 & 82.8 \\
Hybrid BYOL-S ($\alpha_{\text{ss}} = \alpha_{\text{sup}} = 1$)                                                                                          & 66.5 & 75.4 & 90.8 & \textbf{93.8} & \textbf{71.3} & 79.5 & 79.8\\
%Hybrid BYOL-S/CvT                                                                                                                      & 83.8 & 72.5 & 98.3 & 87.5 & 70   & 82.4 \\
Hybrid BYOL-S/CvT ($\alpha_{\text{ss}} = \alpha_{\text{sup}} = 1$)                                                                                      & 78.4 & 74.6 & 99.2 & 83.3 & 66.3 & 80.3 & 82.6 \\
Hybrid BYOL-S/CvT ($\alpha_{\text{ss}} = 1$, $\alpha_{\text{sup}} = 2$)                                                                                   & \textbf{83.8} & 72.5 & 98.3 & 87.5 & 70.0  & \textbf{82.4} & 82.8 \\
  \bottomrule
  \end{tabular}
  \label{tab:2}
\end{table*}

==> Table3_with_WM.tex <==
\begin{table*}[t]
  \centering
  \caption{Impact of hybrid loss weighting (Eq.~\ref{equ:loss}) in \textbf{Hybrid BYOL-S/CvT} pre-training on test UAR (\%).}
  \vspace{-4pt}
  \begin{tabular}{lccccc@{\hspace{20pt}}cc}
  \toprule
    % BYOL:OS loss ratio &
    $\alpha_{\text{ss}}$ : $\alpha_{\text{sup}}$ (Eq.~\ref{equ:loss}) &
    Cog1 & Cog2 & Cog3 & Cog4 & Phys & UM & WM \\
    \midrule
4 : 1              & 73.5          & 71.3          & 97.5          & 87.5          & 60.0          & 77.9 & 80.1 \\
2 : 1              & 72.2          & 72.5          & \textbf{99.2} & \textbf{92.7} & 55.0          & 78.3 & 80.8 \\
4 : 3              & 76.7          & 70.0          & 98.3          & 88.5          & 62.5          & 79.2 & 81.0 \\
1 : 1              & 78.4          & 74.6          & \textbf{99.2} & 83.3          & 66.3          & 80.3 & 82.6  \\
3 : 4              & 80.2          & \textbf{75.0} & \textbf{99.2} & 86.5          & 65.0          & 81.2 & 83.4          \\
1 : 2              & \textbf{83.8} & 72.5          & 98.3          & 87.5          & \textbf{70.0} & \textbf{82.4} & \textbf{83.8}  \\
1 : 4              & 81.4          & 72.5          & 97.9          & 86.5          & 63.8          & 80.4 & 82.4         \\
    \bottomrule
  \end{tabular}
  \label{tab:3}
\end{table*}

